Twisted Equivariant Tate K-Theory

Starting with a $\mathbb{C}^*$-valued cocycle on the global quotient orbifold $X // G$, we apply transgression techniques for 2-gerbes, as developed by Lupercio and Uribe, to construct a gerbe on the orbifold loop space $\mathcal{L}(X//G)$. This gives a loop based definition of twisted equivariant Tate K-theory for finite groups that conforms to the definition that Luecke provides for compact, connected Lie groups. We relate our construction to Ganter's work on Moonshine and Huan's quasi-elliptic cohomology.

==> notes.tex <==


\section{Notes/To-do}

\begin{enumerate}
    \item Tikz up the pictures in loop groupoid section.
    \item Start introduction. Then finish the introduction.
    \item Fiber product notation. [To be added to a notation section in introduction]
    \item Add nomenclature for everything. [Done a bit, not as much as I thought. Questioning how useful a notation index is. Maybe a list of definitions too?]
    \item Prove generalised maps can be represented by an open cover. Ideally without appealing to bibundles, though I suspect this is the cleanest way. [My solution is to move this proof into an appendix on bibundles]
    \item Improve proof of 3.1 - vector bundles only depend on Morita class. [Will be in the bibundles appendix]

    \item Mention how gerbes on a groupoid don't depend groupoid representative. I think this can be reduced to only considering Leray groupoids i.e. choose two Leray descriptions.
    \item Finish bundle gerbe appendix and then clean up the remarks in the gerbe section. [Progress: needs the connective structure part]
    \item Appendix on bibundles? [Yes - I think this is worthwhile as I have two results that are best proven in this context]
    \item Mention why we care about gerbes. This perhaps belongs in the introduction.
    \item Clean up the preamble for the transgression section.
    \item Mention where else the obtained cocycle appears in literature.
    \item Clean up and work on the exposition in last chapter.
    \item Write a section relating my work to Kiran's.
    \item Twisted quasi-elliptic cohomology? Would like to relate to Zhen's work. 
    \item Mention something about the Witten genus and how it takes values in Tate K-theory.
\end{enumerate}

\section{Discussion}

\begin{enumerate}
    \item  What is the best number system for theorem environments? Should, for example, definitions and theorem be numbered separately?
    \item Italicised versus non-italicised theorem environments.
    \item Throughout the ``paper'' or ''thesis''?
\end{enumerate}


\iffalse

Orbifolds are a generalisation of manifolds. Instead of being locally Euclidean, orbifolds are locally a quotient of Euclidean space by a finite group. Initially introduced by Satake in the 1950s under the name V-manifolds, orbifolds were shown to inherit much of the theory from smooth manifolds such as de Rham cohomology, characteristic classes and the Gauss-Bonet theorem. Orbifolds eventually became a prominent subject of interest in fields such as differential topology, geometry and string theory. For a brief overview of the history and applications of orbifolds we recommend the introduction of \cite{orbifoldsandstringytopology}.

In 1997 Moerdijk and Pronk demonstrated how one could view an orbifold as an equivalence class of certain Lie groupoids. This is analogous to representing a manifold by an equivalence class of atlases. In the next section we will define groupoids and the relevant notion of equivalence between them, Morita equivalence. Essentially two groupoids will represent the same groupoid when they are Morita equivalent. We will then describe Moerdijk's notion of a generalised map between orbifolds/groupoids.

Throughout this thesis we tend to use the words orbifold and groupoid interchangeably. The understanding is that when we define a structure on a groupoid this is the same as defining a structure on the orbifold it represents provided there is some invariance under Morita equivalence. For our purposes we mostly only care about the global quotient orbifold $X \mmod G$, but we speak of general orbifolds where possible.

\fi


\begingroup
\addtolength{\jot}{1em}
\begin{align*}
    &\frac{ g(\varphi_2, \Omega_{i+1}, \Theta_{i+1}) \cdot g(\Omega_i, \Theta_i, \varphi_4) }{ g(\Omega_i, \varphi_3, \Theta_{i+1})}
    \times
    \left( \frac{ g( \varphi_1, (\Lambda \cdot \Omega)_{i+1}, \Theta_{i+1}) \cdot g( (\Lambda \cdot \Omega)_i, \Theta_i, \varphi_4) }{g((\Lambda \cdot \Omega)_i, \varphi_3, \Theta_{i+1})} \right)^{-1}\\
    &\hspace{1cm}
        \times \frac{ g(\varphi_1, \Lambda_{i+1}, (\Omega\cdot\Theta)_{i+1}) \cdot g(\Lambda_i, (\Omega\cdot\Theta)_i, \varphi_4) }{g(\Lambda_i, \varphi_2, (\Omega\cdot\Theta)_{i+1})}
        \times \left( \frac{g(\varphi_1, \Lambda_{i+1}, \Omega_{i+1}) \cdot g(\Lambda_i, \Omega_i, \varphi_3) }{g(\Lambda_i, \varphi_2, \Omega_{i+1})}\right)^{-1} \\
    &\hspace{0.5cm}
        = \frac{g(\Lambda_{i+1}, \Omega_{i+1}, \Theta_{i+1})}{g(\varphi_1 \cdot \Lambda_{i+1}, \Omega_{i+1}, \Theta_{i+1})} \times
            \frac{g(\Lambda_i, \Omega_i, \Theta_i\cdot \varphi_4)}{g(\Lambda_i, \Omega_i, \Theta_i)}  \times
            \frac{g(\varphi_2, \Omega_{i+1}, \Theta_{i+1})}{g(\Omega_i, \varphi_3, \Theta_{i+1})}\\
    &\hspace{2cm}
            \times \frac{g(\Lambda_i, \varphi_2, \Omega_{i+1})}{g(\Lambda_i, \Omega_i, \varphi_3)}
            \times \frac{g((\Lambda \cdot \Omega)_i, \varphi_3, \Theta_{i+1})}{g(\Lambda_i, \varphi_2, (\Omega\cdot\Theta)_{i+1})} \\
    &\hspace{0.5cm}
        = \frac{ g(\Lambda_{i+1}, \Omega_{i+1}, \Theta_{i+1}) }{ g(\Lambda_i, \Omega_i, \Theta_i)} 
        \times \frac{g(\Lambda_i, \varphi_2\cdot\Omega_{i+1}, \Theta_{i+1})}{g(\Lambda_i, \Omega_I \cdot \varphi_3, \Theta_{i+1})} \\
    &\hspace{0.5cm}
        = \frac{g(\Lambda_{i+1}, \Omega_{i+1}, \Theta_{i+1})}{g(\Lambda_i, \Omega_i, \Theta_i)}.
\end{align*}
\endgroup


